On-the-fly Code Activation for Attack Surface Reduction

Modern code reuse attacks are taking full advantage of bloated software. Attackers piece together short sequences of instructions in otherwise benign code to carry out malicious actions. Eliminating these reusable code snippets, known as gadgets, has become one of the prime concerns of attack surface reduction. The aim is to break these chains of gadgets, thereby making such code reuse attacks impossible or substantially less common. Previous work on attack surface reduction has typically tried to eliminate such attacks by subsetting the application, e.g. via user-specified inputs, configurations, or features, or by focusing on third-party libraries to achieve high gadget reductions with minimal interference to the application. In this work we present a general, whole-program attack surface reduction technique called OCA that significantly reduces gadgets and has minor performance degradation. OCA requires no user inputs and leaves all features intact. OCA identifies specific program points and through analysis determines key function sets to enable/disable at runtime. The runtime system, thus, controls the set of enabled functions during execution, thereby significantly reducing the set of active gadgets an attacker can use, and by extension, cutting down the set of active gadget chains dramatically. On SPEC CPU 2017, our framework achieves 73.2% total gadget reduction with only 4% average slowdown. On 10 GNU coreutils applications, it achieves 87.2% reduction. On the nginx server it achieves 80.3% reduction with 2% slowdown. We also provide a gadget chain-breaking study across all applications, and show that our framework breaks the shell-spawning chain in all cases.

==> ACM/abstract.tex <==
%%
%% The abstract is a short summary of the work to be presented in the
%% article.
\begin{abstract}
 
foo

\end{abstract}

%%
%% The code below is generated by the tool at http://dl.acm.org/ccs.cfm.
%% Please copy and paste the code instead of the example below.
%%
% \begin{CCSXML}
% <ccs2012>
%   <concept>
%       <concept_id>10011007.10011006.10011041</concept_id>
%       <concept_desc>Software and its engineering~Compilers</concept_desc>
%       <concept_significance>500</concept_significance>
%       </concept>
%   <concept>
%       <concept_id>10010147.10011777</concept_id>
%       <concept_desc>Computing methodologies~Concurrent computing methodologies</concept_desc>
%       <concept_significance>300</concept_significance>
%       </concept>
%  </ccs2012>
% \end{CCSXML}

% \ccsdesc[500]{Software and its engineering~Compilers}
% \ccsdesc[300]{Computing methodologies~Concurrent computing methodologies}

%%
%% Keywords. The author(s) should pick words that accurately describe
%% the work being presented. Separate the keywords with commas.
\keywords{GPU, Scheduler, Compiler}

==> ACM/authors.tex <==
%%
%% The "author" command and its associated commands are used to define
%% the authors and their affiliations.
%% Of note is the shared affiliation of the first two authors, and the
%% "authornote" and "authornotemark" commands
%% used to denote shared contribution to the research.
\author{Chao Chen}
\email{chao.chen@gatech.edu}
\authornote{Both authors contributed equally to the paper}
\affiliation{%
  \institution{Georgia Institute of Technology}
  \city{Atlanta}
  \state{GA}
  \postcode{30332}
}

\author{Chris Porter}
\email{porter@gatech.edu}
\authornotemark[1]
\affiliation{%
  \institution{Georgia Institute of Technology}
  \city{Atlanta}
  \state{GA}
  \postcode{30332}
}

\author{Santosh Pande}
\email{santosh.pande@cc.gatech.edu}
\affiliation{%
  \institution{Georgia Institute of Technology}
  \city{Atlanta}
  \state{GA}
  \postcode{30332}
}

==> IEEE/abstract.tex <==
\begin{abstract}

Code reuse attacks today are taking full advantage
of bloated software.
In this work we load needed functionality
before its point of use and purge it afterward.
We do this on a whole-program basis.
% Unneeded functionality opens
% up avenues for attack, but needed functionality is also
% available for code reuse attacks.
% Prior work has focused on eliminating unneeded
% functionality, or has not been able to do this
% on a whole-program basis.
We build a compiler pass and couple it with a secure
runtime to implement this idea. The results are
promising. (FIXME) On SPEC 2017, our framework achieves
50\% reduction in ROP gadget reduction while suffering
from only 5\% overhead on average.
(FIXME) On coreutils, the numbers are similar: 50\% and 5\%.


% Attack surface reduction through demand driven loading and depends-on program
% properties and control flow



\end{abstract}

\begin{IEEEkeywords}
Compiler, Runtime
\end{IEEEkeywords}

==> IEEE/authors.tex <==
\author{
\IEEEauthorblockN{Chris Porter\textsuperscript{\textsection}}
\IEEEauthorblockA{\textit{Georgia Institute of Technology} \\
Atlanta, USA \\
porter@gatech.edu}
\and
\IEEEauthorblockN{Sharjeel Khan\textsuperscript{\textsection}}
\IEEEauthorblockA{\textit{Georgia Institute of Technology} \\
Atlanta, USA \\
smkhan@gatech.edu}
\and
\IEEEauthorblockN{Girish Mururu}
\IEEEauthorblockA{\textit{Google} \\
Atlanta, USA \\
girishmurore@gmail.com} % FIXME ?
\and
\IEEEauthorblockN{Santosh Pande}
\IEEEauthorblockA{\textit{Georgia Institute of Technology} \\
Atlanta, USA \\
santosh.pande@cc.gatech.edu}
}
